Discovery-Targeted False Discovery Rate Control

In exploratory multiple testing, the false discovery rate (FDR) is a commonly used error criterion, and existing methods typically take an FDR level and return a set of discoveries. However, scientists often begin with a target number of discoveries, and accept any FDR level below a reasonable upper limit. Motivated by this practical need, we develop an FDR control approach with a data-driven, discovery-targeted level, which uses synthetic null p-values to split the p-value information between level selection and multiple testing. For independent p-values, the proposal controls finite-sample FDR given the reported level, which can therefore be interpreted in the standard way of a prespecified level. Asymptotically, the number of discoveries and the reported FDR level converge to the target and the optimal value. We also extend the approach to conformal p-values and to include a null proportion estimate. In simulations and real-data examples, the procedure yields a number of discoveries close to the target and smaller FDR levels compared with methods based on e-values or simultaneous false discovery proportion bounds.

==> generated/v5_figures/brca-seed318/brca-results.tex <==
% Generated by code/run_brca_seed318.py from the saved single run.
With seed 318 and $K=50$, the proposal returns 64 discoveries at reported level 0.2386.
Both e-BH variants and both FDP-bound methods return no discoveries in this run.
The fitted lower-tail source scores are constant in every fold in this run, giving learned e-values equal to one.
Invert BH returns 51 discoveries at level 0.2169, where the BH path jumps across the target, but lacks the conditional FDR guarantee.


==> generated/v5_figures/brca-seed318/brca-table.tex <==
% Generated by code/run_brca_seed318.py from the saved single run.
\begin{table}[!htb]\centering\tablefont
\caption{Breast-cancer analysis at $K=50$ using seed 318: 3170 one-sided Student t-tests and one synthetic null bag with $B=m=3170$.
Reported levels are clipped to $[0.01,0.30]$.
Invert BH is a diagnostic without the conditional FDR guarantee.}
\label{tab:application}
\begin{tabular}{@{}l*{6}{c}@{}}\toprule
Metric & Invert BH & Proposal & \begin{tabular}[c]{@{}c@{}}e-BH\\(learned score)\end{tabular} & \begin{tabular}[c]{@{}c@{}}e-BH\\(fixed score)\end{tabular} & \begin{tabular}[c]{@{}c@{}}FDP bound\\(KR)\end{tabular} & \begin{tabular}[c]{@{}c@{}}FDP bound\\(SC)\end{tabular}\\\midrule
Reported $\widehat q_{50}$ & 0.2169 & 0.2386 & 0.3000 & 0.3000 & 0.3000 & 0.3000 \\
Rejections & 51 & 64 & 0 & 0 & 0 & 0 \\
\bottomrule\end{tabular}
\end{table}


==> generated/v5_figures/protein-seed318/protein-results.tex <==
% Generated by code/run_protein_seed318.py from the saved single partition.
With seed 318 and $K=50$, the observed-null proposal returns 132 discoveries at reported level 0.2404.
Learned-score and fixed-score e-BH return 0 and 13 discoveries, respectively.
Invert BH returns 59 discoveries, and the conformal SC bound returns 0.


==> generated/v5_figures/protein-seed318/protein-table.tex <==
% Generated by code/run_protein_seed318.py from the saved single partition.
\begin{table}[!htb]\centering\tablefont
\caption{PFC2 mouse proteins at $K=50$ using one reference partition with seed 318: 1040 tests, 121 estimation and 300 calibration references.
Reported levels are clipped to $[0.01,0.30]$.
Invert BH is a diagnostic without the conditional FDR guarantee.}
\label{tab:mouse-pfc2}
\begin{tabular}{@{}l*{6}{c}@{}}\toprule
Metric & Invert BH & Proposal & \begin{tabular}[c]{@{}c@{}}e-BH\\(learned score)\end{tabular} & \begin{tabular}[c]{@{}c@{}}e-BH\\(fixed score)\end{tabular} & \begin{tabular}[c]{@{}c@{}}FDP bound\\(KR)$^\dagger$\end{tabular} & \begin{tabular}[c]{@{}c@{}}FDP bound\\(SC)\end{tabular}\\\midrule
Reported $\widehat q_{50}$ & 0.1757 & 0.2404 & 0.3000 & 0.3000 & --- & 0.3000 \\
Rejections & 59 & 132 & 0 & 13 & --- & 0 \\
\bottomrule\end{tabular}
\par\smallskip\begin{minipage}{0.96\linewidth}\footnotesize
$^\dagger$KR is unavailable: shared-calibration conformal p-values are dependent, and distribution-known original p-values are unavailable.
\end{minipage}
\end{table}


==> preamble.tex <==
\usepackage[T1]{fontenc}
\usepackage[margin=1in]{geometry}
\usepackage{amsmath}
\usepackage{newtxtext}
\usepackage[subscriptcorrection]{newtxmath}
\usepackage{graphicx}
\usepackage{booktabs,longtable}
\newcommand{\tablefont}{\small}
\usepackage[round,authoryear]{natbib}
% Retain separate theorem-family counters and the existing proof interface.
\usepackage[amsmath,thmmarks,hyperref]{ntheorem}
\theoremstyle{plain}
\theoremnumbering{arabic}
\theoremheaderfont{\normalfont\bfseries}
\theorembodyfont{\itshape}
\theoremseparator{.}
\theoremsymbol{}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\theorembodyfont{\normalfont}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{step}{Step}
\newtheorem{condition}{Condition}
\newtheorem{property}{Property}
\newtheorem{restrictions}{Restriction}
\newtheorem{example}{Example}
\newtheorem{algo}{Algorithm}
\theoremstyle{nonumberplain}
\theoremheaderfont{\normalfont\itshape}
\theoremsymbol{\ensuremath{\square}}
\newtheorem{proof}{Proof}
\makeatletter
\renewtheoremstyle{nonumberplain}
  {\item[\theorem@headerfont\hskip\labelsep ##1\theorem@separator]}
  {\item[\theorem@headerfont\hskip\labelsep ##1\ ##3\theorem@separator]}
\makeatother
\usepackage[hidelinks]{hyperref}
\usepackage[capitalise,noabbrev]{cleveref}
\hypersetup{pdftitle={Discovery-Targeted False Discovery Rate Control},pdfauthor={Zijun Gao}}
\newcommand{\FDP}{\operatorname{FDP}}
\newcommand{\E}{\mathrm{E}}
\newcommand{\var}{\operatorname{var}}
\newcommand{\ind}{\mathbf{1}}
\newif\ifprintproofs
\bibliographystyle{biometrika}
\newenvironment{keywords}
  {\par\smallskip\noindent\small\textbf{Keywords: }}
  {\par\normalsize\medskip}
\setlength{\floatsep}{16pt plus 2pt minus 2pt}
\setlength{\textfloatsep}{20pt plus 2pt minus 4pt}
\setlength{\intextsep}{16pt plus 2pt minus 2pt}
\setcounter{topnumber}{2}
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{0.8}
\setlength{\emergencystretch}{2em}
\frenchspacing
\raggedbottom


